A probabilistic Weyl law for quantized tori with random potentials

We study the spectrum of the Weyl quantization of complex-valued functions on the torus subject to small perturbations given by random potentials. We prove that the eigenvalues of the perturbed operator satisfy a Weyl law with high probability in the semiclassical limit, extending the results of T. J. Christiansen and M. Zworski (arXiv:0909.2014) and M. Vogel (arXiv:1912.08876).

==> references-compat.tex <==
\makeatletter
\@ifundefined{references@compat@loaded}{%
  \let\references@compat@loaded\@empty
  \def\references@remove@spaces#1{\zap@space#1 \@empty}%
  \def\references@compat@setup{%
    \@ifpackageloaded{biblatex}{%
      \PackageError{references-compat}{This helper requires a BibTeX workflow}%
        {Use the supplied BibTeX setup rather than loading biblatex.}%
    }{%
      \@ifpackageloaded{natbib}{%
        \let\references@original@sort@cites\NAT@sort@cites
        \def\NAT@sort@cites##1{%
          \edef\references@keys{##1}%
          \edef\references@keys{%
            \expandafter\references@remove@spaces\expandafter{\references@keys}}%
          \expandafter\references@original@sort@cites\expandafter
            {\references@keys}%
        }%
      }{%
        \let\references@original@citex\@citex
        \def\@citex[##1]##2{%
          \edef\references@keys{##2}%
          \edef\references@keys{%
            \expandafter\references@remove@spaces\expandafter{\references@keys}}%
          \references@original@citex[##1]{\references@keys}%
        }%
      }%
      \let\references@original@nocite\nocite
      \def\nocite##1{%
        \edef\references@keys{##1}%
        \edef\references@keys{%
          \expandafter\references@remove@spaces\expandafter{\references@keys}}%
        \expandafter\references@original@nocite\expandafter
          {\references@keys}%
      }%
      % Include all original active references before any document citations.
      % An unsorted bibliography style then retains this exact sequence.
      \nocite{%
        Continuous_Potentials_and_Linear_Mass_Distributions,%
        BasakPaquetteZeitouni,%
        BeckerOltmanVogel,%
        BordenaveCapitaineChapon,%
        Probabilistic Weyl Laws for Quantized Tori,%
        DaviesHager,%
        label_1,%
        Dudley,%
        Evans,%
        Gohberg,%
        GuionnetWoodZeitouni,%
        Hager06,%
        HagerSjostrand,%
        HelfferRobert,%
        Lecture notes at the Nordic Summer School,%
        label_2,%
        HormanderSpectral,%
        Ivrii,%
        Jensen Nakamura,%
        Kallenberg,%
        Klenke,%
        label_3,%
        label_4,%
        Mather,%
        label_5,%
        Noel,%
        Distribution of resonances for open quantum maps,%
        Oltman,%
        zeros of holo fct,%
        Sjostrand 2,%
        Sjostrand 3,%
        Sjostr and Vogel 1,%
        SjostrandVogelGeneralToeplitz,%
        Sjostrand and Vogel 2,%
        label_8,%
        Sniady,%
        Random matr theory,%
        label_11,%
        label_9,%
        Weyl,%
        label_12%
      }%
    }%
  }%
  \@ifundefined{AddToHook}{%
    \AtBeginDocument{\references@compat@setup}%
  }{%
    \AddToHook{begindocument/end}{\references@compat@setup}%
  }%
}{}
\makeatother
\endinput

